Structural and compositional properties of brown dwarf disks: the case of 2MASS J04442713+2512164

In order to improve our understanding of substellar formation, we have performed a compositional and structural study of a brown dwarf disk. We present the result of photometric, spectroscopic and imaging observations of 2MASS J04442713+2512164, a young brown dwarf (M7.25) member of the Taurus association. Our dataset, combined with results from the literature, provides a complete coverage of the spectral energy distribution from the optical to the millimeter including the first photometric measurement of a brown dwarf disk at 3.7mm, and allows us to perform a detailed analysis of the disk properties. The target was known to have a disk. High resolution optical spectroscopy shows that it is intensely accreting, and powers a jet and an outflow. The disk structure is similar to that observed for more massive TTauri stars. Spectral decomposition models of Spitzer/IRS spectra suggest that the mid-infrared emission from the optically thin disk layers is dominated by grains with intermediate sizes (1.5micron). Crystalline silicates are significantly more abondant in the outer part and/or deeper layers of the disk, implying very efficient mixing and/or additional annealing processes. Sub-millimeter and millimeter data indicate that most of the disk mass is in large grains (>1mm)

==> photom.tex <==
\begin{center}
\begin{deluxetable}{lcc }
\tablecaption{Photometry \label{photom}}
\tablewidth{0pt}
\tablehead{
\colhead{$\lambda$}      & \colhead{Flux}      & \colhead{Ref.} \\
\colhead{[$\mu$m]}        & \colhead{[mJy]}     & 
}
\startdata
0.43                     & 0.081$\pm$0.022     &       (1)        \\ 
0.55                     & 0.264$\pm$0.068     &       (1)        \\ 
0.7                      & 0.466$\pm$0.096     &       (1)        \\
1.235                    & 21.1$\pm$0.4        &       (2)        \\
1.662                    & 29.3$\pm$0.5        &       (2)        \\
2.159                    & 33.1$\pm$0.5        &       (2)        \\
3.6                      & 44.1$\pm$4.4        &       (3)        \\
4.5                      & 45.5$\pm$4.5        &       (3)        \\
5.8                      & 53.5$\pm$5.3        &       (3)        \\
8.0                      & 70.3$\pm$7.0        &       (3)        \\
8.59                     & 73.9$\pm$7.1        &       (5)        \\
8.99                     & 84.8$\pm$12.0       &       (5)        \\
10.49                    & 97.9$\pm$14.0       &       (5)        \\
%11.25                    & \nodata             &       (5)        \\
%12.81                    & \nodata             &       (5)        \\
%17.65                    & \nodata             &       (5)        \\
%18.72                    & \nodata             &       (5)        \\
24                       & 124.0$\pm$12.4      &       (3)        \\
70                       & 157.0$\pm$15.7      &       (3)        \\
450                      & 36$\pm$15           &       (5)        \\
850                      & 10$\pm$1.5          &       (5)        \\
1300                     & 7.5$\pm$0.89        &       (4)        \\
3470                     & 0.55$\pm$0.12       &       (5)        \\
\enddata
\tablerefs{(1) \citet{2005yCat.1297....0Z}; 
(2) 2MASS;  
(3) \citet{2007A&A...465..855G}; 
(4) \citet{2006ApJ...645.1498S}; 
(5) this work}
\end{deluxetable}
\end{center}

